Non-Parametric Neural Style Transfer

It seems easy to imagine a photograph of the Eiffel Tower painted in the style of Vincent van Gogh's 'The Starry Night', but upon introspection it is difficult to precisely define what this would entail. What visual elements must an image contain to represent the 'content' of the Eiffel Tower? What visual elements of 'The Starry Night' are caused by van Gogh's 'style' rather than his decision to depict a village under the night sky? Precisely defining 'content' and 'style' is a central challenge of designing algorithms for artistic style transfer, algorithms which can recreate photographs using an artwork's style. My efforts defining these terms, and designing style transfer algorithms themselves, are the focus of this thesis. I will begin by proposing novel definitions of style and content based on optimal transport and self-similarity, and demonstrating how a style transfer algorithm based on these definitions generates outputs with improved visual quality. Then I will describe how the traditional texture-based definition of style can be expanded to include elements of geometry and proportion by jointly optimizing a keypoint-guided deformation field alongside the stylized output's pixels. Finally I will describe a framework inspired by both modern neural style transfer algorithms and traditional patch-based synthesis approaches which is fast, general, and offers state-of-the-art visual quality.

==> chapters/06_How.tex <==
\chapter{Details for Improving Style Transfer}
\label{chpt:how}

A pithy description of our proposed algorithm NNST (Chapter \ref{chpt:nnst}) and the early non-parametric neural style transfer algorithm proposed by Chen et al \cite{chen2016fast} would reveal little difference between the two. Both methods explicitly construct a tensor of `target features' by replacing vectors of VGG-derived content features with vectors of VGG-derived style features, then optimize the pixels of the output image to produce the 'target features'. Yet, there is a dramatic difference between the visual quality of the algorithms' outputs. As is often the case, the devil is in the details, and this chapter will explore the important design decisions that can boost a style transfer algorithm's visual quality.

\begin{figure}
    \centering
    \includegraphics{}
    \caption{Visual Comparison between the outputs of Chen et al. \cite{chen2016fast} and a simplified variant of NNST () which uses the feature splitting regime across all scales and does not employ color correction. The primary focus of this section is to explore the which algorithmic details are important for synthesizing the high and middle frequencies of the style image, not on preserving content or replicating the color distribution of the style.}
    \label{fig:chen_nnst_comp}
\end{figure}

==> chapters/NNST/Figures/lynx.tex <==
%% Creator: Inkscape 0.48.3.1, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'lynx.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%%
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{912bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.63777969)%
    \put(0,0){\includegraphics[width=\unitlength]{lynx.pdf}}%
    \put(0.14146107,0.61630217){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{keyframe \#1}}}%
    \put(0.85899121,0.61630217){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{keyframe \#2}}}%
    \put(0.49970703,0.61630217){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{inbetween frame}}}%
    \put(0.13973924,0.0){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{NNST-Opt}}}%
    \put(0.85903749,0.0){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{NNST-Opt}}}%
    \put(0.50152652,0.0){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{Jamri\v{s}ka et al.}}}%
    \Huge
    \put(0.32017544,0.17056695){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{...}}}%
    \put(0.32017544,0.46004064){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{...}}}%
    \put(0.67982456,0.46004064){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{...}}}%
    \put(0.67982456,0.17056695){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{...}}}%
  \end{picture}%
\endgroup%


==> chapters/NNST/Figures/puffin.tex <==
%% Creator: Inkscape 0.48.3.1, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'puffin.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%%
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{2811.96992188bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.31051845)%
    \put(0,0){\includegraphics[width=\unitlength]{chapters/NNST/Figures/puffin.pdf}}%
    \small
    \put(0.18178759,0.30514317){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{style}}}%
    \put(0.47176405,0.30514317){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{content}}}%
    \put(0.68360939,0.30514317){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{NNST-Opt}}}%
    \put(0.89602821,0.34014317){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{NNST-Opt +}}}%
    \put(0.89602821,0.30514317){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{Texler et al.}}}%
  \end{picture}%
\endgroup%


==> chapters/NNST/Related.tex <==
\section{Related Work}\label{sec:related}
Example-based style transfer, non-photorealistic rendering guided by a
single piece of artwork, is a widely studied image synthesis
task. Approaches like our own, in which image synthesis is guided by
explicit matches between spatially localized content and style
features, can be traced to \cite{hertzmann2001image} and related work
on texture synthesis
\cite{efros2001image,efros1999texture,wei2000fast}. Recent patch-based style transfer algorithms have focused on producing extremely high quality outputs when additional human guidance is available, either in the form of edge annotations \cite{lukavc2013painting,lukavc2015brushables}, or specially created style images \cite{fivser2016stylit,benard2013stylizing}. These methods are unified by their use of hand-crafted feature representations and use of nearest neighbors to find content-style correspondences.
%Subsequent extensions of texture synthesis explored alterations to the feature space and image synthesis algorithm in order to improve speed \cite{ashikhmin2003fast}, quality \cite{wu2004feature,kaspar2015self,lee2010directional}, and flexibility \cite{barnes2009patchmatch}. 

\textbf{Optimization-Based Style Transfer: } 
Recent years have marked a significant departure from this line of work, building off techniques introduced by ~\cite{gatys2016image} in `A Neural Algorithm of
Artistic Style'. This work had two major impacts. The first is leveraging
features extracted by a convolutional neural network pretrained for
image classification (typically VGG \cite{simonyan2014very}). The
second is directly optimizing the output's pixels using gradient
descent to simultaneously minimize a `style loss' (typically based on
matching statistics derived from features of the target artwork), and
a `content loss' (typically based on minimizing deviation from the
content image's features). Many works \cite{gatys2016image,berger2016incorporating,li2016combining,risser2017stable,mechrez2018contextual,gu2018arbitrary,kolkin2019style} have proposed alternate style loss formulations, and \cite{kolkin2019style} proposes a relaxed content loss invariant to translations and rotoreflections in feature space.

In the example-based framework, where each style image can be arbitrary and is assumed to be previously unseen, these approaches produce the highest quality output. However, methods that use a content and style loss, both based on VGG features, face a fundamental challenge. In general it is impossible to match the statistics of the style features (satisfying the style loss) while keeping the content features unchanged (satisfying the content loss). Even if the content loss is invariant to rotoreflections \cite{kolkin2019style}, matching the second order statistics captured by the simplest original style loss \cite{gatys2016image,li2017demystifying} generally requires an affine transformation (of which rotoreflections are a subset, and therefore do not provide enough invariance). In practice we observe that content losses based on deep VGG layers tend to cause photographic high frequencies of the original content to bleed into the final output.

To avoid this tension, our proposed algorithm returns to the paradigm of guiding image synthesis with explicitly matched content and style features, although like other NST algorithms we leverage pretrained VGG for feature extraction.

We are not the first to revisit these ideas using neural
features. CNNMRF \cite{li2016combining} replaces the style loss of
\cite{gatys2016image} with minimizing each patch of content feature's
distance from its nearest neighbor patch of style features under the
cosine distance. However, it also regularizes its outputs
using the content loss proposed in \cite{gatys2016image}, leading to
the fundamental tension outlined above. 

We are aware of three similar style transfer works that also explicitly construct a set of target features and do not use a content loss. ~\cite{chen2016fast} take a similar approach to \cite{li2016combining}, but average overlapping feature patches from the style image. This preserves content well, but at the cost of fidelity to the target style. \cite{gu2018arbitrary} add a soft constraint on the matches found by nearest neighbors that each style vector may only be used at most $k$ times, this constraint can be overly restrictive, and overly distorting content. ~\cite{liao2017visual} propose a coarse-to-fine algorithm for finding feature correspondences between the content and style image. Their algorithm produces excellent results on style-content pairs with matching semantics and similar poses (and based on our user study, ink based styles using sparse lines), but generally does not work for more disparate style-content pairs (see Figure \ref{fig:qual_slow}). 

~\cite{Texler20-CAG} also propose a method based on explicit neural feature matching, but to guide an upsampling procedure using patch-based synthesis. Their goal is to increase the resolution of a NST output (such as our own) to 4k resolution and beyond, and their method is complementary to ours.

%\begin{figure}[tp]
%\centering
%\includegraphics[width=\linewidth]{chapters/NNST/Figures/DIA.jpg}
%\begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
%Content & DIA \cite{liao2017visual} & Ours & Style
%\end{tabularx}
%\caption{Deep Image Analogies (DIA) \cite{liao2017visual}, another content loss free method, is designed specifically for style/content pairs with well-matched semantic, and works best when the layout and pose of the two inputs is similar. Our method, along with other generic style transfer methods, is intended to work well even for completely unrelated content/style pairs. We demonstrate our method's greater robustness, applying it to two failure cases from their paper.}
%\label{fig:dia}
%\end{figure}

\begin{figure*}[tp]
\centering
\includegraphics[width=\linewidth]{chapters/NNST/Figures/qual_fast.jpg}
\begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
Content & \cite{Li17} &  \cite{zhang2019multimodal} & \cite{an2021artflow} & NNST-D (Ours) & Style 
\end{tabularx}
\caption{Qualitative comparision between NNST-D and the top three feed-forward methods from our user study, using oil painting, ink, watercolor, and pencil styles. Below each input and result is a zoomed-in portion of the image. While all neural methods to date fail to entirely capture many styles' long range correlation of textural features and high frequency details, our results are dramatically closer than prior work.}
\label{fig:qual_fast}
\end{figure*}

\begin{figure*}[tp]
\centering
\includegraphics[width=\linewidth]{chapters/NNST/Figures/qual_slow.jpg}
\begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
Content & \cite{liao2017visual} & \cite{gatys2016image} & \cite{kolkin2019style} & NNST-Opt (Ours) & Style 
\end{tabularx}
\caption{Qualitative comparision between NNST-Opt and the top three optimization based methods from our user study, using oil painting, ink, watercolor, and pencil styles. Below each input and result is a zoomed-in portion of the image. While all neural methods to date fail to entirely capture many styles' long range correlation of textural features and high frequency details, our results are dramatically closer than prior work.}
\label{fig:qual_slow}
\end{figure*}

%\begin{figure}[tp]
%\centering
%\includegraphics[width=\linewidth]{chapters/NNST/Figures/chen_c.jpg}
%\begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
%Content & Chen \cite{chen2016fast} & Ours & Style
%\end{tabularx}
%\caption{In \cite{chen2016fast} Chen et al.\ also propose a content loss free style transfer method. However, a key difference relative to our method is that they average feature vectors when construction their `target feature tensor'. This helps them preserve content well, but results in failure to capture distinctive elements of the style. We compare our results with theirs on two pairs of inputs taken from their paper.}
%\label{fig:chen}
%\end{figure}

%Other recent work has used optimal transport to find mappings from content features to `stylized' features. In \cite{li2019optimal,mroueh2019wasserstein} the authors find the optimal transport map for the content features under the assumption that the true distribution of content and style features is Gaussian. This is efficient, but limits their stylization to being an affine map applied to the content features. In \cite{kolkin2019style}, Kolkin et al.\ formulate their style loss based on an efficiently computed lower bound on the earth-movers distance. However, like other methods descended from \cite{gatys2016image}, their style loss is fundamentally at odds with the content loss.

\textbf{Universal Feed-Forward Style Transfer: } 
To address the major shortcoming of optimization-based style transfer, its speed, there is a large body of work on training feed-forward methods for `universal style transfer' \cite{Huang17,Li17,chiu2019understanding,yao2019attention,park2019arbitrary,zhang2019multimodal, Chiu2020Iterative,an2021artflow,sheng2018avatar}. Many of these approaches are rooted in closed-form modifications of features extracted from the content image based on the first and second order statistics of the style features \cite{Huang17,Li17,chiu2019understanding}.  \cite{sheng2018avatar} propose a 'style decorator' to hallucinate alternate content features more amenable to stylization. \cite{Chiu2020Iterative} replaces single stage moment matching with an efficient method of iteratively stylizing the content features via analytical gradient descent. \cite{yao2019attention} uses self-attention to improve content preservation in perceptually important regions and \cite{park2019arbitrary} use self-attention to distribute localized style features according to the content's self-similarity. \cite{zhang2019multimodal} improves stylization quality by relaxing the assumption that the feature distributions are uni-modal, and matching clusters of features using a graph cut. \cite{an2021artflow} uses normalizing flows to stabilize style transfer, improving stylization quality and preventing results from changing after multiple rounds of stylization. However, because these methods either must learn to extract information from the style image, or only have access to limited feature statistics, they often struggle to reproduce distinctive elements of the target style. This gives them a disadvantage relative to optimization based methods, which 'learn from scratch' for each new input pair, and consequently the visual quality of feed-forward results is lower. By taking as input a large tensor of rearranged style features extracted by pretrained VGG, NNST-D has direct access to much richer information about the target style.

\textbf{Targeted Feed-Forward Style Transfer: } 
Another common scenario, which we do not address in this work, is when the styles of interest are known beforehand, and a neural network can be pretrained to produce stylizations of the predetermined type(s) \cite{johnson2016perceptual,Zhu17a,junginger2018unpaired,sanakoyeu2018style,kotovenko2019content, svoboda2020two}. These methods are very fast, and can produce high quality results. However, they require enough training data for a given style, and must be retrained for new styles. 


%In addition, while they capture the overall style of an artist, they are generally not well suited to transferring the style of a specific image. Our algorithm is intended for use in the situation where each style image is previously unobserved, and we do not compare to feed-forward methods.
%In addition, XXX. This means that by providing more style vectors than content vectors we can relax the standard optimal transport assumption that the content vectors must be mapped to the entire distribution of the style vectors. This allows us to synthesize the final output without using the style features most incompatible with the content.
%\subsection{Evaluation}
%\nik{Discuss 'Deep Photo Style Transfer's' Evaluation protocol, STROTSS Evaluation protocol, Forsyth evaluation protocol}

%Finding the transformation between content and style features is extremely efficient, and mapping the transformed content features back to pixels only requires a single forward pass through a pre-trained decoder network. There is no fundamental barrier to replacing our pixel optimization with a similarly trained decoder network. However, we have not yet pursued this direction and leave it to future work.


%\begin{figure*}[htp]
%\centering
%\includegraphics[width=\linewidth]{chapters/NNST/Figures/alpha_resub.pdf}
%\caption{visualization of the method's content/style tradeoff caused by varying $\alpha$. Because our final output is synthesized entirely based on features from the style image, there is non-trivial stylization even when $\alpha=0$}
%\label{fig:alpha}
%\end{figure*}


==> chapters/STROTSS/Related.tex <==
\newcommand{\qCIm}[3]{\includegraphics[height=#3\textwidth]{chapters/STROTSS/Figures/Compare/#1_#2} }

\newcommand{\qCRow}[2]{\qCIm{#1}{Content}{#2} & \qCIm{#1}{Style}{#2} & \qCIm{#1}{Ours}{#2} & \qCIm{#1}{Reshuffle}{#2} & \qCIm{#1}{Gatys}{#2} & \qCIm{#1}{CNNMRF}{#2} & \qCIm{#1}{Contextual}{#2} }

\begin{figure}
	\centering
	
	\begin{tabular}{ccccccc}
	\qCRow{00}{0.13}\\
	\qCRow{01}{0.06}\\
	\qCRow{02}{0.13}\\
	\qCRow{03}{0.07}\\
	\qCRow{04}{0.13}\\
	\qCRow{05}{0.13}\\
	Content & Style & Ours & Reshuffle \cite{gu2018arbitrary} & Gatys \cite{gatys2016image} & CNNMRF \cite{li2016combining} & Contextual \cite{mechrez2018contextual} 
\end{tabular}



	\caption{Qualitative comparison between our method and prior work. Default hyper-parameters used for all methods}
	\label{fig:comp_fig}
\end{figure}




\section{Related Work}\label{sec:related}

Style transfer algorithms have existed for decades, and traditionally
relied on hand-crafted algorithms to render an image in fixed style
\cite{haeberli1990paint,hertzmann1998painterly}, or 
hand-crafting features to be matched between an arbitrary style to the content image
\cite{hertzmann2001image,efros2001image}. The
state-of-the-art was dramatically altered in 2016 when Gatys et
al.~\cite{gatys2016image} introduced Neural Style Transfer. This
method uses features extracted from a neural network pre-trained for
image classification. It defines style in terms of the Gram matrix of
features extracted from multiple layers, and content as the feature
tensors extracted from another set of layers. The style loss is
defined as the Frobenius norm of the difference in Gram
feature matrices between the output image and style image. The content
loss is defined as the Frobenius norm of the difference between
feature tensors from the output image and the style image. Distinct
from the framework of Neural Style Transfer, there are several recent
methods \cite{liao2017visual, Aberman2018} that use similarities
between deep neural features to build a correspondence map between the
content image and style image, and warp the style image onto the
content image. These methods are extremely successful in paired
settings, when the
contents of the style image and content image are similar, but are not
designed for style transfer between arbitrary images (unpaired or
texture transfer).

Subsequent work building upon \cite{gatys2016image} has explored
improvements and modifications along many axes. Perhaps the most
common form of innovation is in proposals for quantifying the 'stylistic similarity' between two images~\cite{li2016combining, berger2016incorporating, risser2017stable, mechrez2018contextual}. For example in order to capture long-range spatial dependencies Berger et al.~\cite{berger2016incorporating} propose computing multiple Gram matrices using translated feature tensors (so that the outer product is taken between feature vectors at fixed spatial offsets). Both~\cite{gatys2016image} and~\cite{berger2016incorporating} discard valuable information about the complete distribution of style features that isn't captured by Gram matrices.

In~\cite{li2016combining} Li et al. formulate the style loss as
minimizing the energy function of a Markov Random Field over the
features extracted from one of the latter layers of a pretrained CNN,
encouraging patches (which yielded the deep features) in the target
image to match their nearest neighbor from style image in feature
space. Other functionally similar losses appear
in~\cite{risser2017stable}, which treats style transfer as matching
two histograms of features, and~\cite{mechrez2018contextual}, which
matches features between the style and target which are significantly
closer than any other pairing. In all of these methods, broadly speaking,
features of the output are encouraged to
lie on the support of the distribution of features extracted from the
style image, but need not cover it. These losses are all similar to
one component of the Relaxed EMD ($R_A$). However, our method differs
from these approaches because our style term also encourages covering
the entire distribution of features in the style image ($R_B$). Our
style loss is most similar in spirit to that proposed by Gu et
al~\cite{gu2018arbitrary}, which also includes terms that encourage
fidelity and diversity. Their loss minimizes the distance
between explicitly paired individual patches, whereas ours minimizes the distance between
distributions of features. 

Another major category of innovation is replacing the
optimization-based algorithm of~\cite{gatys2016image} with a
neural network trained to perform style transfer, enabling real-time
inference. Initial efforts in this area were constrained to a limited
set of pre-selected styles~\cite{johnson2016perceptual}, but
subsequent work relaxed this constraint and allowed arbitrary styles
at test time~\cite{huang2017arbitrary}. Relative to slower
optimization-based methods these works made some sacrifices in the
quality of the output for speed. However, Sanakoyeu et
al.~\cite{sanakoyeu2018styleaware} introduce a method for
incorporating style images from the same artist into the real-time
framework which produces high quality outputs in real-time, but in
contrast to our work relies on having access to multiple images with
the same style and requires training the style transfer mechanism separately for each new style.

Various methods have been proposed for controlling the output of style
transfer. In~\cite{gatys2017controlling} Gatys et al. propose two
'global' control methods, that affect the entire output rather than a
particular spatial region. One method is decomposing the image into
hue, saturation, and luminance, and only stylizes the luminance in
order to preserve the color palette of the content image. A second
method from~\cite{gatys2017controlling} is to generate an auxiliary
style image either to preserve color, or to transfer style from only a
particular  scale (for example the transferring only the brush-strokes, rather than the larger and more structurally
complex elements of the style). These types of user control are
orthogonal to our method, and can be incorporated into it.

Another type of control is spatial, allowing users to ensure that certain regions of the output should be stylized using only features from a manually selected region of the style image (or that different regions of the output image should be stylized based on different style images). In~\cite{gatys2017controlling, lu2017decoder} the authors propose forms of spatial control based on the user defining matched regions of the image by creating a dense mask for both the style and content image. We demonstrate that it is straightforward to incorporate this type of user-control into our formulation of style transfer. In the supplement we show an example comparing the spatial control of our method and ~\cite{gatys2017controlling}, and demonstrate that both yield visually pleasing results that match the spatial guidance provided.

\begin{figure}[!tbh]
	\centering
	\includegraphics[width=0.9\textwidth]{chapters/STROTSS/Figures/figure_guidance_small.jpg} 
	\caption{Examples of using guidance for
          aesthetic effect (left, point-to-point)) and error
          correction (right, region-to-region). In the top row the
          images are arranged in order of content, output,
          style. Below each content and style image we show the
          guidance mask, and between them the guided output.}
	\label{fig:control_fig}
\end{figure}

\newcommand{\cKIm}[3]{\includegraphics[height=#3cm]{chapters/STROTSS/Figures/content_knob/#1_#2}}

\newcommand{\contentKnobRow}[2]{\cKIm{#1}{c}{#2} & \cKIm{#1}{2000}{#2} & \cKIm{#1}{1000}{#2} & \cKIm{#1}{0500}{#2} & \cKIm{#1}{0250}{#2} & \cKIm{#1}{s}{#2}}



\begin{figure}[tb]
	\centering
\begin{tabular}{cccccc}
	\contentKnobRow{pollen}{2.6}\\
	\contentKnobRow{dome}{2.6}\\
	Content & $\alpha=32.0$ & $\alpha=16.0$ & $\alpha=8.0$ & $\alpha=4.0$ & Style
\end{tabular}\vspace{-.5em}
	\caption{Effect of varying $\alpha$, the content loss weight, on our unconstrained style transfer output, because we stylize at four resolutions, and halve $\alpha$ each time, our default $\alpha=16.0$ is set such that $\alpha=1.0$ at the final resolution.}
	\label{fig:knob_fig}
\end{figure}




Evaluating and comparing style transfer algorithms is a challenging
task because, in contrast to object recognition or segmentation, there
is no established ``ground truth'' for the output. The most common
method is a qualitative, purely subjective comparison between the
output of different algorithms. Some methods also provide more refined
qualitative comparisons such as texture
synthesis~\cite{risser2017stable,gu2018arbitrary} and
inpainting~\cite{berger2016incorporating}. While these comparisons
provide insight into the behavior of each algorithm, without
quantitative comparisons it is difficult to draw conclusions about the
algorithm's performance on average. The most common quantitative
evaluation is asking users to rank the output of each algorithm
according to aesthetic appeal~\cite{gu2018arbitrary, li2018closed,
  mechrez2017photorealistic}. Recently Sanakoyeu et
al.~\cite{sanakoyeu2018styleaware} propose two new forms of
quantitative evaluation. The first is testing if an neural network
pretrained for artist classification on real paintings can correctly
classify the artist of the style image based on an algorithm's
output. The second is asking experts in art history which algorithm's
output most closely matches the style image. We designed our human
evaluation study, described in section \ref{sec:h_eval}, to give a
more complete sense of the trade-off each algorithm makes between
content and style as its hyper-parameters vary. To the best of our knowledge it is the first such effort.




\newcommand{\xfig}[1]{\includegraphics[height=1.6cm]{chapters/STROTSS/Figures/Qual_Cross/#1}}
\newcommand{\xfigLine}[1]{\xfig{#1} & \xfig{#1_01} & \xfig{#1_05} & \xfig{#1_03} & \xfig{#1_04} & \xfig{#1_02}}
\newcommand{\xfigLineS}[1]{ & \xfig{s01} & \xfig{s05} & \xfig{s03} & \xfig{s04} & \xfig{s02}}


==> front_materials/dedication.tex <==
To my grandparents
